Policy Message Passing: A New Algorithm for Probabilistic Graph Inference

A general graph-structured neural network architecture operates on graphs through two core components: (1) complex enough message functions; (2) a fixed information aggregation process. In this paper, we present the Policy Message Passing algorithm, which takes a probabilistic perspective and reformulates the whole information aggregation as stochastic sequential processes. The algorithm works on a much larger search space, utilizes reasoning history to perform inference, and is robust to noisy edges. We apply our algorithm to multiple complex graph reasoning and prediction tasks and show that our algorithm consistently outperforms state-of-the-art graph-structured models by a significant margin.

==> puzzle_table_vg.tex <==
\begin{table}[h!]
\centering
  \begin{tabular}{c c c c c c c c c c}
  \toprule
     \multicolumn{1}{c}{Models} & \multicolumn{3}{c}{Accuracy(\%)} & \multicolumn{3}{c}{Kendall-tau}
    \\ \hline
    & 3x3 & 4x4 & 6x6 & 3x3 & 4x4 & 6x6
    \\
    \hline
    random & 11.11 & 6.25 & 2.78 & - & - & -
    \\
    GNN & 82.83 & 72.46 & 61.22 & 85.47 & 79.94 & 79.58
    \\
    GNN-attention & 86.87 & 77.35 & 71.27 & 88.75 & 85.51 & 83.35
    \\
    RRN & 85.60 & 77.27 & 69.23 & 88.07 & 83.31 & 78.50
    \\
    NRI & 87.63 & 73.51 & 70.62 & 89.37 & 80.06 & 79.91
    \\
    \hline
    PMP (ours)& \textbf{97.92} & \textbf{96.74} & \textbf{94.61} & \textbf{98.58} & \textbf{98.07} & \textbf{97.05}
    \\ \bottomrule
    \end{tabular}
  \caption{Performance results on Visual Genome dataset, measured by per-patch classification accuracy and correlation score Kendall-tau.  Results are shown across different puzzle sizes.}
  \label{tbl:vg}
\end{table}

==> temp.tex <==

\begin{figure}[t]
\hspace{-10mm}
\begin{subfigure}{0.65\textwidth}
  \begin{tabular}{c c c c c c c c c c}
  \toprule
     \multicolumn{1}{c}{Models} & \multicolumn{3}{c}{Accuracy(\%)} & \multicolumn{3}{c}{Kendall-tau}
    \\ \hline
    & 3x3 & 4x4 & 6x6 & 3x3 & 4x4 & 6x6
    \\
    \hline
    random & 11.11 & 6.25 & 2.78 & - & - & -
    \\
    GNN & 82.83 & 72.46 & 61.22 & 85.47 & 79.94 & 79.58
    \\
    GNN-attention & 86.87 & 77.35 & 71.27 & 88.75 & 85.51 & 83.35
    \\
    RRN & 85.60 & 77.27 & 69.23 & 88.07 & 83.31 & 78.50
    \\
    NRI & 87.63 & 73.51 & 70.62 & 89.37 & 80.06 & 79.91
    \\
    \hline
    PMP & \textbf{97.92} & \textbf{96.74} & \textbf{94.61} & \textbf{98.58} & \textbf{98.07} & \textbf{97.05}
    \\ \bottomrule
    \end{tabular}
  \caption{Performance results on Visual Genome dataset, measured by per-patch classification accuracy and correlation score Kendall-tau.  Results are shown across different puzzle sizes.}
  \label{tbl:vg}
\end{subfigure}\hspace{16mm}%
\begin{subfigure}{0.3\textwidth}
  \includegraphics[width=1.0\textwidth]{figs/Analysis.pdf}
  \caption{Analysis of our model on number of inference steps and number of functions.}
  \label{fig:analysis}
  \end{subfigure}
\caption{Performance on Visual Genome(left) and model analysis plots(right).}
\label{fig:vg_result}
\end{figure}
%\vspace{-5mm}
